Differentiable Tree Operations Promote Compositional Generalization

In the context of structure-to-structure transformation tasks, learning sequences of discrete symbolic operations poses significant challenges due to their non-differentiability. To facilitate the learning of these symbolic sequences, we introduce a differentiable tree interpreter that compiles high-level symbolic tree operations into subsymbolic matrix operations on tensors. We present a novel Differentiable Tree Machine (DTM) architecture that integrates our interpreter with an external memory and an agent that learns to sequentially select tree operations to execute the target transformation in an end-to-end manner. With respect to out-of-distribution compositional generalization on synthetic semantic parsing and language generation tasks, DTM achieves 100% while existing baselines such as Transformer, Tree Transformer, LSTM, and Tree2Tree LSTM achieve less than 30%. DTM remains highly interpretable in addition to its perfect performance.

==> sections/submission/abstract.tex <==
\begin{abstract}
In the context of structure to structure transformation tasks, sequences of discrete symbolic operations (e.g.,  op codes or programs) are an important but difficult to learn tool due to their non-differentiability. To support learning sequences of symbolic operations, we propose a differentiable tree interpreter which compiles high-level symbolic tree operations into subsymbolic matrix operations on tensors. We introduce a novel Differentiable Tree Machine (\blackboard) architecture which combines our interpreter with an external memory and an agent which learns to sequentially select tree operations to perform a desired transformation.
%in a fully differentiable environment, we propose compatible with Supervised Learning, we propose a novel step-wise predictor/interpreter architecture, utilizing an external memory to hold multiple Tensor Product Representations (TPRs) to simulate the accumulated effect of a sequence of weighted blends of operations on a structure.  Our structure for this paper is a binary tree and each TPR in the memory holds a weighted blend of binary trees.
On synthetic supervised tree-to-tree transduction tasks, we demonstrate that our approach achieves drastically better compositional generalization and interpretability than baselines such as the Transformer and LSTM.
\end{abstract}





%\begin{abstract} Discrete symbolic operations are important for working with structured objects but are difficult to learn due to their non-differentiability. Using binary trees as an example, we propose using the Tensor Product Representation (TPR) to encode a factorized distribution of structured objects in vector space. We develop several systematic discrete operations which can be represented as linear transformations on underlying TPR trees. Since the structured objects are represented as activation vectors and the discrete operations are represented as linear transformations, our proposal is fully differentiable. We introduce a novel \blackboard architecture which learns to sequentially read, manipulate, and write binary trees or distributions of them using an external memory. \roland{we should include here a high-level description of overall architecture that uses this external memory}. On synthetic supervised tree-to-tree translation tasks, we demonstrate that our approach achieves drastically better compositional generalization and interpretability compared to baselines such as the Transformer and LSTM. \end{abstract

==> sections/submission/discussion.tex <==
\section{Conclusions, Limitations, and Future Work}

We introduce \blackboard, an architecture for leveraging differentiable tree operations and an external memory to achieve compositional generalization. Our trees are embedded in vector space as TPRs which allow us to perform symbolic operations as differentiable linear transformations. \blackboard\ outperforms baselines across a variety of synthetic tree-to-tree tasks and is highly interpretable.

The major limitation of \blackboard\ is that the input and output must be structured as trees. Future work will focus on allowing \blackboard\ to take in unstructured data, generate a tree, and then perform the operations we described. This will allow \blackboard\ to be evaluated on a larger variety of datasets. Our hope is that \blackboard\ will be able to scale to language modeling and other large pretraining tasks.

Another hurdle for \blackboard\ is the size of trees that it can handle. The encoding scheme we presented here requires the depth of possible trees to be determined beforehand so that the appropriate number of roles can be initialized. Additionally, while the TPR dimension grows linearly with the number of nodes in a tree, the number of nodes in a tree grows exponentially with depth. The majority of \blackboard\ parameters reside in $W_{shrink}$ the linear transformation from TPR space to model space. This can cause memory issues when representing deep trees. We leave methods for extending to an unbounded depth and lossy compression of the role space to future work.

The sequences of all possible operations defines an infinite set of functions which are linear transformations. \blackboard\ reduces the operation space to individual transformations, but it may be feasible for a model to learn more expressive functions which combine multiple \car, \cdr, and \cons\ operations in a single step. Future work will investigate other tree functions such as Tree Adjoining Grammars as well as other data structures.

==> sections/submission/impact.tex <==
\section{Impact Statement}
To our knowledge, the work presented here does not pose any societal harms beyond the scope of general AI research. As with all ML research, there is a risk that improvements in ML  technologies could be used for harmful purposes. We hope that the interpretability offered by our method can contribute to an understanding of neural network models to increase controllability as well as improve and verify fairness.

==> sections/submission/introduction.tex <==
\section{Introduction}
Symbolic manipulation is a hallmark of human reasoning \cite{Newell1980PhysicalSS, newell1982knowledge}. Reasoning in the symbolic space through discrete symbolic operations can result in better out-of-distribution generalization and increased interpretability. However, learning to directly manipulate discrete symbolic structures remains challenging, even though modern deep learning has made significant advances in representation learning. One key issue is that discrete symbolic operations are non-differentiable and thus not amenable to learning via gradient methods. Continuous representations offer more powerful learning capacity --- but this capacity often comes at the expense of interpretability and compositional generalization.

\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{images/fig1m.pdf}}
\caption{A high level overview of our model which consists of three modules. The Neural Tree Agent is a learnable neural network which, at each step of processing, selects the operation to perform and the arguments over which to operate. The Differentiable Tree Interpreter is an analytical function which compiles high level symbolic operations into subsymbolic matrix operations on tensors. The output of the interpreter is a blended tree which is written to Tree Memory and the process repeats. The final tree written to memory is the output tree. }
\label{fig:high-level}
\end{center}
\vskip -0.2in
\end{figure}

Tensor Product Representation (TPR) is a general encoding of structured symbolic objects in vector space \cite{Smolensky1990TensorPV}.
TPR decomposes a symbolic object into a set of role-filler pairs, e.g., a position in a tree (the role) and the label for that position (the filler of that role). Within each pair, the role and the filler are represented using vectors and are bound together using the tensor product operation. 
%We show in \textsection \ref{tpr} that the TPR space is able to encode a family of factorized distributions over symbolic structures. In addition, we can take linear combinations of TPRs to interpolate among such distributions.

In this work, we focus our attention on binary trees and three Lisp operators: \car, \cdr, and \cons\ \cite{steele1990common} (otherwise known as left-child, right-child, and construct new tree). Examples of the three operations are shown in Figure \ref{fig:car-cdr-cons}. Crucially, within the TPR space, these symbolic operators on discrete objects become linear operators on continuous vectors. Unlike normal symbolic structures, the vector space nature of TPRs allows us to blend multiple symbolic structures as interpolations between classic discrete structures.%, making them amenable to learning via backpropogation. 
%This enables new super-symbolic capacities, such as blending %discrete 
%operators and arguments, while still maintaining an interpretable %linearly-structured 
%representation space. %As these continuous representations are differentiable, we can learn a powerful nonlinear parameterization of the operators' decision space.
We restrict processing over our TPR encodings to the interpretable linear operations implementing the three Lisp operators and their interpolations; this computation is differentiable and therefore accessible to backpropogation. Gradients can run through our differentiable tree operations so that we can optimize the sequencing and blending of linear operations using nonlinear deep learning models.

Using TPRs to represent binary trees, we design a novel Differentiable Tree Machine architecture, \blackboard\footnote{Code available at publication.} (\textsection \ref{sec:model}), which can systematically manipulate binary trees. At each step of computation, \blackboard\ soft-selects  a binary tree to read from an external memory, soft-selects a linear operator to apply to the tree, and then writes the resulting tree to a new memory slot. Soft-selecting among a set $S$ of $n$ elements in a vector space here means: computing a vector $w \in \mathbb{R}^n$ of non-negative weights that sum to one, and returning the sum of the elements in $S$ weighted by $w$ (i.e., $w \cdot S$). 
 As the learning progresses, the weights on the operators tend to become 1-hot and the continuous blends of trees become more discrete as we converge to a discrete sequence of operations for each sample. 
  We validate our proposal empirically on a series of synthetic tree-to-tree datasets that test a model's ability to generalize compositionally (\textsection \ref{sec:empirical}).

The \blackboard\ architecture achieves near perfect out-of-distribution generalization for the examined synthetic tree-transduction tasks on which standard models exhibit partial or no out-of-distribution generalization. 

Overall, our contributions include:

\begin{itemize}
  \item A novel \blackboard\ architecture for interpretable, continuous manipulation of blended binary trees.
  \item Four datasets to test out-of-distribution generalization on binary tree-to-tree tasks.
  \item Empirical comparison of \blackboard\ and baselines on these datasets which demonstrates the unique advantages of \blackboard\ in terms of compositional generalization and interpretability.
\end{itemize}

\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{images/car-cdr-cons.png}}
\caption{An example showing how each of our three operations function.}
\label{fig:car-cdr-cons}
\end{center}
\vskip -0.2in
\end{figure}

==> sections/submission/model.tex <==
\section{Differentiable Tree Machine (\blackboard) Architecture for Binary Tree Translation} \label{sec:model}

\begin{figure*}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\textwidth]{images/layer.png}}
\caption{Step 1 of the \blackboard\ architecture is expanded to show the information flow in \blackboard. The yellow boxes show which parameters are learnable. The blue box highlights the Neural Tree Agent, and the green boxes highlight components in tree space, the Differentiable Tree Interpreter (Eq 1) and Tree Memory. The left side of the Neural Tree Agent is a standard transformer layer with self-attention and a feedforward network. Residual connections and layer norm are not shown.}
\label{architecture}
\end{center}
\vskip -0.2in
\end{figure*}

\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{images/staircase.png}}
\caption{Inputs to the Neural Tree Agent at each step of processing \paul{TODO: the words in the boxes should be changed from token to encoding.}}
\label{step}
\end{center}
\vskip -0.2in
\end{figure}

In order to actualize the theory described in Section \ref{tpr}, we introduce the Differentiable Tree Machine (\blackboard), a model that is capable of learning how to perform operations over binary trees. Since the primitive functions \car, \cdr, and \cons\ are precomputed at initialization from the orthogonally generated role vectors, this learning problem reduces to learning which operations to perform on which trees in Tree Memory to arrive at a correct output. A high-level overview of our model is given in Figure \ref{fig:high-level}. \blackboard\ consists of a learned component (Neural Tree Agent), a differentiable pre-designed tree interpreter described in Equation \ref{eq:output}, and an external Tree Memory for storing trees.

At a given timestep $l$, our agent selects the inputs to Equation \ref{eq:output}: the tree arguments for the operations ($\vec{T}^{(l)}$), the new root symbol for \cons\ ($s^{(l)}$) and how much to weight the output of each operation ($\vec{w}^{(l)}$). To select $\vec{T}^{(l)}$, \blackboard\ produces coefficients over the trees in Tree Memory, where the coefficients across trees in $\vec{T}^{(l)}$ sum to 1. For example, if Tree Memory contains only $T_0\ \&\  T_1$, weights $\vec{a}^{(l)}_{\car} = (a^{(l)}_{\car,0}, a^{(l)}_{\car,1})$ are computed to define the argument to \car:
$T_{\car}^{(l)}=a^{(l)}_{\car,0}T_0 + a^{(l)}_{\car,1}T_1$,
and similarly for \cdr\ and the two arguments of \cons.  $\vec{a}^{(l)}_{T}=(\vec{a}^{(l)}_{\car};\vec{a}^{(l)}_{\cdr};\vec{a}^{(l)}_{\cons 0};\vec{a}^{(l)}_{\cons 1})$ denotes all such weights.


These decisions are computed within the Neural Tree Agent module of \blackboard\ using a standard Transformer layer consisting of multiheaded self-attention, a feedforward network, residual connections, and layer norm. Figure \ref{architecture} shows the computation in a single step of \blackboard. Figure \ref{step} show the input to this Transformer over multiple time steps. When a binary tree is read from Tree Memory, it is compressed from the TPR dimension $d_tpr$ to the Transformer input dimension $d\_model$ using a linear transformation $W_{shrink} \in \mathbb{R}^{d\_tpr \times d\_model}$. We also feed in two special tokens to encode the operation-weighting coefficients and the new root-symbol prediction. In addition to the standard parameters in a Transformer layer, our model includes three additional weight matrices $W_{op} \in \mathbb{R}^{d\_model \times 3}$, $W_{root} \in \mathbb{R}^{d\_model \times d\_symbol}$, and $W_{arg} \in \mathbb{R}^{d\_model \times 4}$. $W_{op}$ projects the operation token encoding into logits for the three operations which are then normalized via softmax. $W_{root}$ projects the root symbol token encoding into the new root symbol. \paul{Go through a make sure we converge on a singular use of filler or symbol instead of using both interchangeably. Filler is okay to use in the TPR section.} $W_{arg}$ projects the encoding of each TPR in memory to logits for the four tree arguments, the input to \car, \cdr, and \cons\ left and right. The arguments for each operator are a linear combination of all the TPRs in memory, weighted by the softmax of the computed logits. These values are used to create the output for this step as described in equation \ref{eq:output} and the output TPR is written into Tree Memory.  For the beginning of the next step, the contents of the Tree Memory are encoded to model dimension by $W_{shrink}$ and appended to the Neural Tree Agent Transformer input sequence.  The input to the Neural Tree Agent Transformer grows by one compressed tree encoding at each time step to incorporate  the newly produced tree, as shown in Figure \ref{step}.

The tree produced by the final step of our network is used as the output (predicted tree). We minimize the mean-squared error between the predicted symbol at each node in the predicted tree and the ground-truth tree. Additional training details can be found in Section \ref{sec:blackboard-training}.
%\pasha{I'm convinced this is the same as the squared distance between the final (non-discretized) TPR and the target TPR, with no unbinding of fillers needed --- because of the orthonormality of the role vectors.}


==> sections/submission/related_work.tex <==
\section{Related Work}

\subsection{Compositional Generalization}
Research on compositional generalization has been one of the core issues in Machine Learning since its inception. Despite improvements in architectures and scalability \cite{csordas2021devil}, neural network models continue to have difficulty with out-of-distribution generalization \cite{najoung}. The lack of robust compositional generalization has been a central argument against neural networks as models of cognition for almost half a century %(who should I cite, Fodor and Pylysh?) 
by proponents of GOFAI systems which leverage symbolic structures \citep[e.g.][]{fodor1988connectionism,marcus2003algebraic}. These symbolic systems are brittle and have scalability problems %with regards to learning 
due to their incompatibility with differentiable methods of learning. Our work attempts to bridge the neural network-symbolic divide by placing symbolic systems in vector space where a first-order gradient can be derived as a learning signal. 

%\kate{could explain difference between lexical and structural generalization here, to contextualize our OOD evaluation results}

In practice, the term ``compositional generalization" has been associated with a range of different tasks \citep{hupkes2020compositionality}. \citet{kim-linzen-2020-cogs} identify a key distinction relevant to natural language: lexical versus structural generalization. \emph{Lexical} generalization is required when a model encounters a primitive (e.g. a word) in a structural environment (e.g. a position in a tree) where it has not been seen during training. %, such as the JUMP split of the SCAN dataset \citep{lake2018generalization}. \citet{patel-etal-2022-revisiting} show that simple training data manipulations enable standard seq-to-seq models such as Transformer and LSTM to solve the JUMP split. 
\citet{najoung} demonstrate that lexical generalization is not yet fully solved: pretrained language models still do not consistently generalize fully novel lexical items. \emph{Structural} generalization is required when a model encounters a structure which was not seen during training, such as a longer sentence or syntactic tree with new nodes. The tasks we study below explicitly test both types of compositional generalization (\textsection \ref{sec:datasets}).

Our proposed \blackboard\ model encodes and manipulates data exclusively in the form of Tensor Product Representations (TPRs; \textsection \ref{sec:TPR}). This formalism inherently supports composition and decomposition through symbol-role bindings, creating an inductive bias toward symbolic operations. \emph{Lexical} generalization is straightforward when syntactic trees are encoded as TPRs: a novel symbol can easily bind to any role.  \emph{Structural} generalization is possible through our linear representation of the \car, \cdr, and \cons \ functions, as these operators are not sensitive to the size or structure of the trees they take as arguments.
We evaluate \blackboard's capacity for both types of compositional generalization in \textsection \ref{sec:results}.

\subsection{Tensor Product Representations (TPRs)} \label{sec:TPR}

Tensor Product Representations have been used to increase performance and interpretability across textual question-answering \cite{schlag2018learning, palangi2018question}, natural-language-to-program-generation \cite{chen}, math problem solving \cite{imanol}, synthetic sequence tasks \cite{mccoy2018rnns, soulos2020discovering}, summarization \cite{jiang2021enriching}, and translation \cite{soulos2021structural}. While previous work has focused on using TPRs to structure and interpret representations, the processing over these representations was done using black-box neural networks. In this work, we predefine structural operations to process TPRs and use black-box neural networks to parameterize the information flow and decision making in our network. 

\subsection{Differentiable Computing}
One approach to integrating neural computation and GOFAI systems is Differentiable Computing. In this approach, components of symbolic computing are re-derived in continuous and fully differentiable manners to allow learning with backpropogation. In particular, neural networks which use an external memory have received considerable attention \cite{Graves2014NeuralTM, Graves2016HybridCU, Weston2014MemoryN, nram}.

Another important aspect of Differentiable Computing is integrating structured computation graphs into neural networks. Tree-LSTMs \cite{tai-etal-2015-improved} use parse trees to encode parent nodes in a tree from their children's representations. Tree Transformers \cite{wang-etal-2019-tree} modify standard multi-headed attention to integrate tree information into the attention computation. \paul{Add citations and explanations of the other tree transformer and transformer grammar}. Neural Module Networks \cite{Andreas2015NeuralMN} are a separate differentiable computing paradigm where functions in a symbolic program are replaced with black-box neural networks. 

A few works have explored using differentiable interpreters to learn subfunctions from program sketches and datasets \cite{bosnjak17a, Reed2015NeuralP}. Most similar to our work, \citet{Joulin2015InferringAP, Grefenstette2015LearningTT} learn an RNN which can leverage a stack including discrete push and pop operations in a differentiable manner. While they use a structured object to aid computation, the operations they perform are simply read/write operations over unstructured vectors whereas the operations we deploy in this work are structured operations over vectors with embedded structure.

%\roland{I am just searching for "differentiable simulators" and see several papers, e.g., https://arxiv.org/abs/2202.00817; we should probably acknowledge this area of work here (mostly differentiable physics simulators for RL);}



%\subsection{Program synthesis}

%\subsection{Learning to Manipulate Symbolic Objects}
%\paragraph{GOFAI}
%\paragraph{LSTM/Tranformer}
%\edward{e.g., Berkeley tree-to-tree paper, tree transformer}
%\paragraph{Reinforcement Learning}
%\edward{neural turing machine paper}

==> sections/submission/results.tex <==
\section{Empirical Validation} \label{sec:empirical}

\begin{table*}[ht]
\label{tab:results}
\vskip 0.15in
\begin{center}
\begin{sc}
\begin{tabular}{lcccc}
\toprule
Data set & \blackboard\ & Transformer & LSTM & GRU \\
\midrule
\textbf{car\_cdr\_seq}\\
 -train & $0.9480 \pm 0.04$ & 1.0000 ± 0.00 & 1.0000 ± 0.00 & 0.9954 ± 0.00 \\
 -test IID & $0.9500 \pm 0.04$ & 1.0000 ± 0.00 & 1.0000 ± 0.00 & 0.9983 ± 0.00  \\
 -test OOD lexical & \textbf{0.9440 ± 0.04} & 0.7582 ± 0.00 & 0.7596 ± 0.00 & 0.7569 ± 0.00 \\
 -test OOD structural & \textbf{0.9340 ± 0.04} & 0.6972 ± 0.02  & 0.4253 ± 0.10 & 0.4407 ± 0.06 \\
\textbf{Active$\leftrightarrow$Logical} & & &  \\
 -train &  1.0000 ± 0.00 & 1.0000 ± 0.00 & 1.0000 ± 0.00 & 1.0000 ± 0.00  \\
 -test IID &  1.0000 ± 0.00& 1.0000 ± 0.00 & 1.0000 ± 0.00 & 1.0000 ± 0.00 \\
-test OOD lexical &  \textbf{1.0000 ± 0.00} & 0.3116 ± 0.00 & 0.3132 ± 0.00 & 0.3132 ± 0.00 \\
-test OOD structural &   \textbf{1.0000 ± 0.00} & 0.0000 ± 0.00 & 0.0000 ± 0.00  & 0.0000 ± 0.00 \\
\textbf{Passive$\leftrightarrow$Logical} & & &  \\
 -train & 1.0000 ± 0.00 & 1.0000 ± 0.00 & 1.0000 ± 0.00 & 1.0000 ± 0.00 \\
 -test IID &  1.0000 ± 0.00 & 1.0000 ± 0.00 & 1.0000 ± 0.00 & 1.0000 ± 0.00 \\
-test OOD lexical &   \textbf{1.0000 ± 0.00} & 0.3636 ± 0.00 & 0.3651 ± 0.00 & 0.3650 ± 0.00 \\
-test OOD structural &   \textbf{1.0000 ± 0.00} & 0.0000 ± 0.00 & 0.0000 ± 0.00 & 0.0116 ± 0.01  \\
\textbf{Active \& Passive$\rightarrow$Logical} & & &  \\
 -train & 1.0000 ± 0.00 & 1.0000 ± 0.00 & 1.0000 ± 0.00 & 1.0000 ± 0.00 \\
 -test IID & 1.0000 ± 0.00 & 1.0000 ± 0.00 & 1.0000 ± 0.00 & 1.0000 ± 0.00 \\
 -test OOD lexical &   \textbf{1.0000 ± 0.00} & 0.3203 ± 0.00 & 0.3217 ± 0.00 & 0.3237 ± 0.00 \\
-test OOD structural &   \textbf{1.0000 ± 0.00} & 0.0000 ± 0.00 & 0.0000 ± 0.00 & 0.0000 ± 0.00 \\
\bottomrule
\end{tabular}
\end{sc}
\end{center}
\vskip -0.1in
\caption{Mean accuracy and standard deviation across 5x random initializations on synthetic tree-to-tree transduction tasks using different model architectures. Test sets include in-distribution and out-of-distribution splits.}
\end{table*}

\subsection{Datasets} \label{sec:datasets}
\paul{consider adding a figure with some examples from the datasets to help people understand what the transformation is.}
We introduce the \textbf{Basic Sentence Transforms} dataset for testing tree-to-tree transformations.\footnote{Data available at publication.} It contains various synthetic tree-transform tasks, including a Lisp function interpreter task and several natural-language tasks inspired by semantic parsing and language generation. It is designed to test compositional generalization in structure transformations, as compared to most existing compositionality-related datasets, which are designed for linear sequence transformations.

Each task in the dataset has five splits: train, validation, test, out-of-distribution lexical (ood-lexical), and out-of-distribution structural (ood-structural). The ood-lexical split tests a model's ability to perform zero-shot lexical generalization to new adjectives not seen during training.  The ood-structural split tests a model's structural generalization by using longer adjective sequences and new tree positions not seen during training. The train split has 10,000 samples; all of the other splits have 1250 samples. Samples of these tasks can be found in Appendix B. We focus our evaluation on the following four tasks:

\textbf{CAR-CDR-SEQ} is tree transformation task where the source tree represents a template-generated English sentence and the target tree represents a subset of the source tree.  The target tree is formed from a sequence of Lisp \car\ and \cdr\ operations on the source tree.  The desired sequence of operations is encoded into a single  token in the source tree root, and the transformation requires learning how to interpret this root token and execute the associated sequence of actions.  The token is formed according to the Lisp convention for combining these operations into a single symbol (starting with a $\mathtt{c}$, followed by the second letter of each operation, and terminated by an $\mathtt{r}$, e.g., $\mathtt{cdaadr}$ denotes the operation sequence: \cdr, \car, \car, \cdr). This task uses sequences of 1-4 \car/\cdr\ operations (resulting in 30 unique functions).

\textbf{Active$\leftrightarrow$Logical} contains syntax trees in active voice and logical form. Transforming from active voice into logical form is similar to semantic parsing, and going from logical form to active voice is common in natural language generation.

\textbf{Passive$\leftrightarrow$Logical}
contains syntax trees in passive voice and logical form. This task is similar to the one above but is more difficult and requires more operations. The passive form also contains words that are not present in logical form, so unlike Active$\leftrightarrow$Logical, the network needs to insert additional nodes. At first glance, this does not seem possible with \car, \cdr, and \cons; we will show how our network manages to solve this problem in an interpretable manner in \textsection \ref{sec:interpret}. The input and output of Figure \ref{fig:high-level} show a transformation from logical form to passive form.

\textbf{Active \& Passive$\rightarrow$Logical} contains input trees in either active or passive voice and output trees in logical form. This tests whether a model can learn to simultaneously parse different trees into a shared logical form.

\subsection{Baseline Architectures}
For our baseline models, we linearize our trees by coding them as a left-to-right sequences with parentheses to mark the tree structure.

\paragraph{Transformer}
For our Transformer model, we use the PyTorch library implementation of the Encoder-Decoder Transformer \cite{vaswani}.  We search over model and training hyperparameters and choose the combination that has the highest (and in the case of ties, quickest to train) mean validation accuracy on the Active \& Passive$\rightarrow$Logical task. The best hyperparameter setting was then used to train models on all four of our tasks.  More training details can be found in Appendix A. 

\paragraph{GRU and LSTM}
For our GRU and LSTM models, we use  GRU \cite{cho-etal-2014-properties} and LSTM \cite{Hochreiter1997LongSM} seq2seq \cite{sutskever} implementations that support hyperparameters for attention (on/off), bidirectionality (on/off), and the number of encoder and decoder layers.  We search over model and training hyperparameters and choose the combination that has the highest (and in the case of ties, quickest to train) mean validation accuracy on Active \& Passive$\rightarrow$Logical. The best hyperparameter setting was then used to train models on all four of our tasks.  More training details can be found in Appendix A. 

%\paragraph{TreeLSTM} Our TreeLSTM model... Put some results here as preliminaries... (dev scores) TreeLSTM+attention on CAR-CDR-RCONS 41.0, CAR-CDR-CONS 43.6

%\roland {One other interesting baseline we could include is the "simple agent" from the original BB which operates on the same TPR source tree.  When it is able to be trained, it's OOD is not strong, similar to our other baselines.  In this case, it shows the value of symbolic operations vs. unstructured ops}


\subsection{Results} \label{sec:results}
The results for \blackboard\ and the baselines can be seen in Table \ref{tab:results}. \blackboard\ runs achieve 100\% accuracy  across all splits for three of the four tasks, and for some of the runs in the  \textbf{CAR\_CDR\_SEQ} task. While the baselines perform similarly to \blackboard\ when compared on train and test iid, the results are drastically different when comparing the results across OOD splits. Across all datasets, \blackboard\ generalizes similarly regardless of the split, whereas the baselines struggle with with lexical generalization and fail completely at structural generalization.

The baseline models perform the best on \textbf{CAR\_CDR\_SEQ}, whereas this is the most difficult task for \blackboard. We suspect that tuning the hyperparameters for \blackboard\ directly on this task would alleviate the less-than-perfect performance. Despite performing less than perfectly, \blackboard\ performance on the OOD splits of \textbf{CAR\_CDR\_SEQ} outperforms all of the baselines.

Whereas \textbf{CAR\_CDR\_SEQ} involves identifying a subtree (or subsequence for the baselines) within the input, the other four tasks involve reorganizing the input and potentially adding additional tokens in the case of \textbf{Passive$\leftrightarrow$Logical}. The baselines seem capable of some lexical generalization, but they are not able to solve any of the structural generalization samples. This is in line with research showing that current models struggle much more with structural generalization than lexical generalization \cite{najoung}.

\begin{comment}
vs RL methods
- Baselines:
    - Vanilla Policy Gradient and Proximal Policy Optimization
        - with TPR state encoding vs Tree LSTM/RNN or Transformer state encoding
        - with 0-1 reward vs TPR reward
- Datasets:
    - Car/Cdr/Seq (key experiment, PPO might work just as fine)
    - Active logical  (key experiment, PPO might not work?)
- Claims:
    - TPBB performs better or learns faster if all methods achieve a perfect performance;
    - TPBB performance exhibits a lower variance;
    - TPR state encoding and/or TPR reward might help the RL baselines
    - (optional) sample-efficiency and compositional generalization: a priori, there are no reasons for RL to do better or worse



- TPBB exhibits better compositional generalization;
- TPBB is more sample-efficient.


TODO: how sample efficient can our model be?
\end{comment}

\begin{figure}[]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{images/interpret.png}}
\caption{An interpretable transformation from logical form to passive. The interpretation is discussed in Section \ref{sec:interpret}. \paul{Regenerate these trees to make them sharper and use full triangles for subtrees where we don't represent the entire tree.}}
\label{fig:interpret}
\end{center}
\vskip -0.2in
\end{figure}

\subsection{Interpreting Inference as Programs} \label{sec:interpret}
The output of the Neural Tree Agent at each timestep can be interpreted as routing data and performing a predefined operation. At convergence, we find that the path from the input tree to the output tree is defined by interpretable one-hot softmax distributions. For the \textbf{CAR-CDR-SEQ} task, our model learns to act as a program interpreter and performs the correct sequence ($\sim$94\% accuracy) of operations on subsequent trees throughout computation. For the language tasks, we can trace the program execution to see how the input tree is transformed into the output tree. An example of our model's behavior can be seen in Figure \ref{fig:interpret}. In particular, we were excited to find an emergent operation in our model's behavior. Transducing from Logical$\rightarrow$Passive not only requires rearranging nodes but also inserting new words into the tree, ``was" and ``by". At first glance, \car, \cdr, and \cons\ do not appear to support adding a new node to memory. The model learns that taking \cdr\ of a tree with only a single child returns an empty tree (the third step in Figure \ref{fig:interpret}); the empty tree can then be used as the inputs to \cons\ in order to write a new word as the root node with no children on the left or right (the fourth step). The programmatic nature of our network at convergence --- the fact that the weighting coefficients $\vec{w}, \vec{a}$ become 1-hot --- makes it trivial to discover how an undefined operation emerged during training.

==> sections/submission/theory.tex <==
\section{Differentiable Tree Operations} \label{tpr}

A completely general formalization of compositional structure is defined by a set of roles, and an instance of a structure results from assigning these roles to particular fillers \cite{Newell1980PhysicalSS}. Intuitively, a role characterizes a position in the structure, and its filler is the substructure that occupies that position. 

In this work, we use a lossless encoding for structure in vector space. Given a tree depth limit of depth $D$, the total number of  tree nodes is $N=(b^{D+1}-1)/(b-1)$ where $b$ is the branching factor. We generate a set of $N$ orthonormal role vectors of dimension $d_r=N$. For a particular position in a tree $r_i$, a filler $f_i$ is assigned to this role by taking the outer product of the filler vector and role vector $f_i \otimes r_i$. The value of the entire structure is the sum over the individual filler-role combinations $T = \sum_i f_i \otimes r_i$. Since the role vectors are orthonormal, a filler $f_i$ can be recovered from $T$ by the inner product between $T$ and $r_i$, $f_i = Tr_i$.

Moving forward, we will focus on the case of binary trees ($b = 2$), which serve as the foundation for a substantial amount of symbolic AI research. From the orthonormal role set, we can generate matrices to perform the Lisp operators \car, \cdr, and \cons. 
For a tree node reached from the root by following the path $x$, denote its role vector by $r_x$; e.g., $r_{011}$ is the role vector reached by descending from the root to the left (0th) child, then the right (1st) child, then the right (1st) child.
In order to extract the subtree which is the left child of the root (Lisp \car), we need to zero out the root node and the right child subtree while moving each filler in the left subtree up one level. Extracting the right subtree (Lisp \cdr) is a symmetrical process. This can be accomplished by:

$\car(T)\!=\!\underline{D}_0 T$;
$\cdr(T)\!=\!\underline{D}_1 T$;
$\underline{D}_c \!=\! I_F \! \otimes \! \sum_{x \in \underline{P}} r_{x}r_{cx}^T$

where $I$ is the identity matrix on filler space and $\underline{P}$ is the set of all paths from the root down to depth less than $D$.

Lisp \cons\ constructs a new binary tree given two trees to embed as the left- and right-child. In order to add a subtree as the $c$th child of a new root node, we define $\underline{E_c}$ to add $c$ to the top of the path-from-the-root for each position:

$\cons(T_0,T_1)=\underline{E}_0 T_0 + \underline{E}_1 T_1$;
$\underline{E}_c = I_F \otimes \sum_{x \in \underline{P}} r_{cx}r_x^T$

 When performing \cons, a new filler $s$ can be placed at the parent node of the two subtrees $T_0$ and $T_1$ by adding $s \otimes r_{root}$ to the output of \cons.
Our model uses linear combination to blend the results of applying the three Lisp operations. The output of step $l\in1:L$, when operating on the arguments $\vec{T}^{(l)}=(T_{\car}^{(l)},T_{\cdr}^{(l)},T_{\cons 0}^{(l)},T_{\cons1}^{(l)})$, is\:

\begin{equation} \label{eq:output}
\begin{split}
O^{(l)}(\vec{w}^{(l)}, \vec{T}^{(l)}, s^{(l)}) = w^{(l)}_\car \car(T_{\car}^{(l)}) + w^{(l)}_\cdr \cdr(T_{\cdr}^{(l)}) \\ + w^{(l)}_\cons \left( \cons(T_{\cons0}^{(l)}, T_{\cons1}^{(l)}) +  s^{(l)} \otimes r_{root} \right)
\end{split}
\end{equation}

%\begin{align} 
%\begin{split}
%O^{(l)}(\vec{w}^{(l)}, \vec{T}^{(l)}, s^{(l)}) = & \; w^{(l)}_\car \car(T_{\car}) + w^{(l)}_\cdr \cdr(T_{\cdr}) \\
%& + w^{(l)}_\cons \left( \cons(T_{\cons0}, T_{\cons1}) +  s^{(l)} \otimes r_{root} \right)
%\end{split}
%\end{align}

The three operations are weighted by the level-specific weights $\vec{w}^{(l)} = (w^{(l)}_\car,  w^{(l)}_\car, w^{(l)}_\cons)$, which sum to 1.

